vLSM: Low tail latency and I/O amplification in LSM-based KV stores

LSM-based key-value (KV) stores are an important component in modern data infrastructures. However, they suffer from high tail latency, in the order of several seconds, making them less attractive for user-facing applications. In this paper, we introduce the notion of compaction chains and we analyse how they affect tail latency. Then, we show that modern designs reduce tail latency, by trading I/O amplification or require large amounts of memory. Based on our analysis, we present vLSM, a new KV store design that improves tail latency significantly without compromising on memory or I/O amplification. vLSM reduces (a) compaction chain width by using small SSTs and eliminating the tiering compaction required in L0 by modern systems and (b) compaction chain length by using a larger than typical growth factor between L1 and L2 and introducing overlap-aware SSTs in L1. We implement vLSM in RocksDB and evaluate it using db_bench and YCSB. Our evaluation highlights the underlying trade-off among memory requirements, I/O amplification, and tail latency, as well as the advantage of vLSM over current approaches. vLSM improves P99 tail latency by up to 4.8x for writes and by up to 12.5x for reads, reduces cumulative write stalls by up to 60% while also slightly improves I/O amplification at the same memory budget.

==> Makefile <==
TARGET=paper
FILES = $(wildcard *.tex) Makefile

all: $(TARGET).pdf

$(TARGET).pdf: $(FILES) $(FIGS)  $(TARGET).bbl
	-pdflatex -shell-escape $(TARGET)
	-bibtex $(TARGET)
	-pdflatex -shell-escape $(TARGET)
	-pdflatex -shell-escape $(TARGET)

$(TARGET).bbl: $(TARGET).bib
	-bibtex $(TARGET)

results: FORCE clean_results
	cd results/overlap-without-all-stats && echo "Echo cded into results dirs" && \
	../../scripts/pdf-cdf.py && cd ..&&\
	cd sst-overlap && echo "Echo cded into results dirs" && \
	../../scripts/pmf-cdf.py

clean_results:
	-rm -f results/overlap-without-all-stats/overlap1/*.pdf
	-rm -f results/overlap-without-all-stats/overlap2/*.pdf
	-rm -f results/overlap-without-all-stats/overlap4/*.pdf
	-rm -f results/sst-overlap/uniform/*.pdf
	-rm -f results/sst-overlap/ycsb-zipfian/*.pdf

view:
	pkill -9  evince || true
	evince $(TARGET).pdf > /dev/null &

clean:
	rm -f *.out *.cut *.aux *.bbl *.log *.blg *.ent $(TARGET).pdf 

all_clean: clean
	latexmk -C

up:	update

update:
	-git status
	-git pull

cc: clean commit

commit:
	-git status
	-git commit -m "text modification" -a
	git push

status:
	git status

commiti:
	git status
	-git commit -a
	-git push

lastdiff2:
	-git diff --name-status HEAD HEAD~2

lastdiff:
	-git diff --name-status HEAD HEAD~1

aspell:
	aspell --lang=en --mode=tex check file.tex

FORCE:


==> discuss.tex <==
\section{Discussion}

We note that there appear to be interesting variations of our variable-size-SST technique:
%
(a) One could create vSSTs on a different level, e.g., between two levels on the device. We believe this is less preferable to
creating vSSTs in the first level on the device ($L_2$ in our case) because it allows high-cost vSSTs to leave longer until they
are re-shuffled from other compactions. High-cost vSSTs in smaller levels are re-shuffled by necessity more frequently, e.g., if
each memtable is merged with the full $L_1$ then each such compaction re-creates vSSTs, providing a new opportunity for low-cost
vSSTs to appear.
%
(b) We could consider applying the same technique in multiple levels of the KV store. Although this looks interesting, it is unclear how we should use vSSTs as the source for creating new vSSTs on the next level and what the effect will be. It would appear
that this would quickly lead to vSSTs of reasonably small size, below any low threshold meant to guard constant overheads in the
design of the KV store.

We believe tail latency can benefit significantly from further reduction of SST size. RocksDB is not necessarily the right platform
for this, given that it exhibits high constant overheads, e.g., for re-creating guards during compactions by using an array copy
operation or managing recovery via a manifest that is flushed after each compaction. \note{ab: check} We leave for future work the
use of vSSTs in KV store designs that exhibit lower constant overheads than RocksDB and are more appropriate for reducing further
the size of SSTs below 2-4 MB and in the order of tens or hundreds of KBs.

We believe that device throughput is an interesting parameter that can change the design of KV stores, even for tail latency
purposes. Storage devices with throughput in the order of 10 GBytes/s have already appeared~\cite{leisnvme,nvmemilops} and technology trends
indicate that device throughput will keep increasing, as this is mostly an issue of parallelism at various levels within each
device and within the server that hosts multiple devices. Therefore, we can assume that KV stores will be limited by CPU. In such
a context, it is interesting to explore how excess device throughput and limited CPU availability can be combined with \name{} to
further reduce tail latency. \note{ab:check.would be nice to make it a bit more specific.}


